A Theory of Second-Order Wireless Network Optimization and Its Application on AoI

This paper introduces a new theoretical framework for optimizing second-order behaviors of wireless networks. Unlike existing techniques for network utility maximization, which only considers first-order statistics, this framework models every random process by its mean and temporal variance. The inclusion of temporal variance makes this framework well-suited for modeling stateful fading wireless channels and emerging network performance metrics such as age-of-information (AoI). Using this framework, we sharply characterize the second-order capacity region of wireless access networks. We also propose a simple scheduling policy and prove that it can achieve every interior point in the second-order capacity region. To demonstrate the utility of this framework, we apply it for an important open problem: the optimization of AoI over Gilbert-Elliott channels. We show that this framework provides a very accurate characterization of AoI. Moreover, it leads to a tractable scheduling policy that outperforms other existing work.

==> ge_model_case.tex <==
\section{A Special Case: Gilbert-Elliot Model} \label{sec:ge model}

Obtaining the explicit expressions for $\Bar{w}_i$ and $v_i$ is difficult for non-I.I.D channel, thus it is also difficult for $\mu_{\{S\}}$ and $\sigma_{\{S\}}^2$ while channels are independent with each other. 
In this paper, we study a simple Markovian model to obtain explicit expressions as a special case.
% special case
We consider the 2-state Markov approach as the Gilbert-Eliot model by Gilbert \cite{Gilbert1960GEmodel} and Elliot \cite{Elliot1963GEmodel} in Figure [xxx]. 
For each flow $i$, its connection process follows the Gilbert-Elliot model with a good (G) state and a bad (B) state, which represents the connection is ON and OFF respectively. 
The transition matrix $A$ is given as follow: 
\begin{align*}
    p_i &= Prob\{W_i(t) = 0|W_i(t-1) = 1\}\\
    r_i &= Prob\{W_i(t) = 1| W_i(t-1) = 0\}\\
    A_i &= \begin{pmatrix} 1-p_i & p_i \\ r_i & 1-r_i \end{pmatrix}.
\end{align*}  
Following the idea of Hablinger and Hohlfeld \cite{Gilbert1960GEmodel}, we can calculate the mean $T\Bar{w}_i$ and variance $Tv_i$ for any consecutive time slots $T$ via the generating functions. 
Specifically, we have:
\begin{align}
    T\Bar{w}_i &= (T+1)\frac{r_i}{p_i + r_i}\\
    Tv_i &= \frac{2Tr_i^2+Tp_ir_i}{(p_i+r_i)^2}  + \frac{2p_ir_i(1-p_i-r_i)}{(p_i+r_i)^3}T \notag \\ &\qquad- \frac{2p_ir_i((1-p_i-r_i)^2-(1-p_i-r_i)^{T+2})}{(p_i+r_i)^4}.
\end{align} The deviation can be found in Appendix []. 
